sec-certs: Examining the security certification practice for better vulnerability mitigation

Products certified under security certification frameworks such as Common Criteria undergo significant scrutiny during the costly certification process. Yet, critical vulnerabilities, including private key recovery (ROCA, Minerva, TPM-Fail...), get discovered in certified products with high assurance levels. Furthermore, assessing which certified products are impacted by such vulnerabilities is complicated due to the large amount of unstructured certification-related data and unclear relationships between the certified products. To address these problems, we conducted a large-scale automated analysis of Common Criteria certificates. We trained unsupervised models to learn which vulnerabilities from NIST's National Vulnerability Database impact existing certified products and how certified products reference each other. Our tooling automates the analysis of tens of thousands of certification-related documents, extracting machine-readable features where manual analysis is unattainable. Further, we identify the security requirements that are associated with products being affected by fewer and less severe vulnerabilities. This indicates which aspects of certification correlate with higher security. We demonstrate how our tool can be used for better vulnerability mitigation on four case studies of known, high-profile vulnerabilities. All tools and continuously updated results are available at https://seccerts.org

==> abstract.tex <==
\begin{abstract}
Products certified under security certification frameworks such as Common Criteria undergo significant scrutiny during the costly certification process. Yet, critical vulnerabilities, including private key recovery (ROCA, Minerva, TPM-Fail...), get discovered in certified products with high assurance levels. Furthermore, assessing which certified products are impacted by such vulnerabilities is complicated due to the large amount of unstructured certification-related data and unclear relationships between the certificates.
To address these problems, we conducted a large-scale automated analysis of Common Criteria and FIPS 140 certificates. We trained unsupervised models to learn which vulnerabilities from NIST's National Vulnerability Database impact existing certified products and how certified products reference each other. Our tooling automates the analysis of tens of thousands of certification-related documents, extracting machine-readable features where manual analysis is unattainable. Further, we identify the security requirements that are associated with products being affected by fewer and less severe vulnerabilities (on average). This indicates which aspects of certification correlate with higher security. We demonstrate how our tool can be used for better vulnerability mitigation on four case studies of known, high-profile vulnerabilities.
All tools and continuously updated results are available at \url{https://seccerts.org} \anon{(web content anonymized)}.

\end{abstract}


%To capture relationships between certificates that affect the impact of vulnerabilities we built a graph of references between certificates.

%, timely notification of affected product end-user.

%We extracted a reference graph of more than 10 thousand items certified under the Common Criteria (CC) and FIPS 140 schemes and 
%, also to steer the current search for more lightweight certification schemes like EUCC \cite{eucc, fips_cav} that aim to decrease certification time and cost by simplifying and automating (parts of) the certification process.


%%%%%%%%%%%%%%%%%% Old abstract %%%%%%%%%%%%%%%%%% 
\if0
We performed a large-scale automated analysis of Common Criteria and FIPS 140 certificates that provided us with a data-based insight into more than two decades of the certification ecosystem and allows for automated vulnerability notification of users of (potentially) vulnerable products. In doing so, we identified many hurdles which impede such automatic analysis and can be addressed by our provided list of recommendations.

We extracted a reference graph of more than 10 thousand items certified under the Common Criteria (CC) and FIPS 140 schemes and trained a classifier (\evalCcPrecision{} precision) for pairing certified products with the corresponding entries in the NIST National Vulnerability Database. Unsupervised classifier allows predictions on newly introduced (future) certificates and/or discovered vulnerabilities, timely notification of end-user and was qualitatively evaluated using five past high-profile vulnerabilities. 

The text-based temporal and spatial analysis reveals many insights into the certification ecosystem: \texttt{AVA\_VAN} (vulnerability analysis) and \texttt{ALC\_TAT} (tools and techniques) security assurance requirements (SARs) have the largest negative correlation with the number and severity of the paired vulnerabilities. The majority of certificate maintenance updates that are subsequent to exposed vulnerabilities do not address these vulnerabilities explicitly. Standardized cryptographic algorithms are relatively slowly introduced in certified products. All tools and continuously updated results are available at \url{https://seccerts.org}.
\fi

==> acknowledgments.tex <==
\section{Acknowledgments}\label{sec:ack}


This work was supported and funded by the following institutions and grants.  The Internal grant agency of MUNI, CZ.02.2.69/0.0/0.0/19\_073/0016943, RedHat Czech, Cyber Security Network of Competence Centres for Europe - CyberSec4Europe, Tools for AI-enhanced Security Verification of Cryptographic Devices (AI-SecTools), Cyber-security Excellence Hub in Estonia and South Moravia (CHESS).

==> background.tex <==
\section{Background}
\label{sec:background}

%This section describes the certification background of the Common Criteria framework. 
%For completeness, we also describe the  FIPS 140 certification framework in Appendix~\ref{sec:appendix_fips}. 

In the CC certification standard \cite{cc}, any security-related product can be certified with the primary focus 
%of the certification is 
being the development process. The main assumption is that if the process is correct, the products will most likely be secure. 
Before certification, the applicant needs to choose a set of Security Functional Requirements (SFR) and Security Assurance Requirements (SAR) that the Target of Evaluation (ToE) aims to adhere to. 
%Preferably, 
Usually, the applicant chooses from an already established list of Protection Profiles (PP) that bind typical use cases (e.g., smartcards) to their usual SFR and SAR specifications. 
During the certification, an independent evaluator, usually an independent laboratory, verifies the product's conformance to this specification. 
Depending on the chosen Protection Profile, 
%of security requirements, 
the product can be certified on multiple Evaluation Assurance Levels (EAL) \cite{cc_overview_2017}, where usually higher EALs provide higher confidence (they also come at a higher cost) that the security features are reliably implemented. 

Within the CC framework, the certification process is performed by many national CC Certificate Authorizing Schemes, and the certification is based on the security evaluation conducted by accredited security laboratories.

For our automated analysis, we use the following documents that accompany the CC certification process and are publicly available:
\begin{description}[noitemsep]
\item[Security Target] -- provided by the applicant to the evaluation facility, specifies the certified product, including the protection profile, SFR, and SAR. 
\item[CSV/HTML web pages]with additional metadata and summary documents automatically generated by the CC portal \cite{cc_webpage} or portals of Certificate Authorizing Schemes. 
\item[Certification Report] -- issued by the certification scheme (e.g., US NIAP) after evaluation by an accredited evaluation facility (e.g., Acumen Security), contains a summary of the certification results.
\item[Certificate] -- issued by the certification scheme, including the most important information, e.g, ToE name and the obtained EAL.
\item[Maintenance Report(s)] -- documenting smaller changes in an already certified product that do not require a full re-certification.
\item[Protection Profile(s)] -- template for a specific class of products, created either by a single vendor or, more commonly, in collaboration \cite{pp_colab}.
\end{description}

We combine the information 
%coming 
from the aforementioned documents with publicly available information about vulnerabilities. 
In particular, the NVD enriches CVE vulnerability records by, among others, 
%things, 
connecting vulnerabilities to their vulnerable Common Platform Enumeration (CPE) records \cite{nvd_cpe}. The CPE records aim to fingerprint the product configuration (vendor, product name, version, 
%target 
hardware, etc.) and are manually assigned to NVD-listed vulnerabilities. 
%We also use these records in our automated analysis. 

==> conclusions.tex <==
\section{Conclusions and future work}
\label{sec:conclusions}

The evaluation labs responsible for the security certification of products are in a conflict of interest as they are paid by vendors. This incentivises them to certify products that should not otherwise pass the certification process. This issue has already been recognized by Cohney et. \cite{DBLP:conf/ccs/CohneyGH18} who noted that it was one of the reasons for NIST moving away from the \enquote{independent test lab} model. Together with non-transparent certification often based on proprietary documents and procedures, this undermines the credibility of the whole certification ecosystem. 

To assist the stakeholders of Common Criteria, we turned the existing certification artifacts into a machine-processable dataset, paired the certificates with NVD, and reconstructed the full graph of inter-certificate references. By doing so, we gained an insight into various attributes of the CC certificates that span over 25 years. This increases transparency and accountability of the whole certification. Better, we allow the stakeholders to fast and precise impact assessment of vulnerabilities that may affect products of their interest.

We demonstrated that higher rigor in certification requirements -- as conveyed by Security Assurance Requirements (SAR) -- is associated with a \emph{lower} number and \emph{less severe} vulnerabilities for the majority of examined SAR classes. Further, to display the effectiveness of our tool in vulnerability assessment, we revisited four major incidents that struck CC-certified products. The \texttt{sec-certs} tool proved invaluable during such analysis, leading to the identification of many additional vulnerable products, and considerably reducing the time required for the analysis. 

Finally, we deliver a web presentation with weekly updated results of our work, providing the stakeholders with easy access to analyzed certification artifacts and to notifications about newly discovered vulnerabilities that may impact them. This will help to ensure that stakeholders are informed of the latest developments and can make informed decisions about the products they use. The whole toolchain can also be self-hosted and enriched with additional -- potential non-public information -- for stronger security analysis. 

As future work, we envision natural language processing as a valuable tool to extract security-relevant information from the certification artifacts. Cohney et al.~\cite{DBLP:conf/ccs/CohneyGH18} already showed that one can identify vulnerable products only by manually searching for alerting phrases in their text specification, and we believe that such task could be automated and outsourced to recent NLP models. Additionally, NLP models could automatically identify the context of the references between the certified products, or even identify non-certified dependencies (e.g., included cryptographic library). With such ability at hand, it would be possible to more closely analyze the threats to the ecosystem of certified products. Further, we consider expanding our analysis also to EMVCo~\cite{emvco} artifacts.

%In conclusion, our research provides databased highlighting the importance of transparency and accountability in the certification process to ensure the security of products and to prevent conflicts of interest that may compromise it. 


% \begin{itemize}
%     \item (Note: Current version of conclusions mostly talk about web tool, not highlighting research outputs.)
%     \item The evaluation labs are in the conflict of interests as they are paid by a vendor and are therefore incentivized to let certify  products that should not be otherwise passed. As Cohey \cite{DBLP:conf/ccs/CohneyGH18} notes, this conflict was one of the reasons that NIST moved away from the `independent test lab' model.
%     \item Turning certificates into machine-processable datasets, providing insight into certificate ecosystem evolution since 1997.
%     \item Real-world impact assesment of certification requirements rigour as expressed by SAR's levels. Recommendation for future certification updates.
%     \item The tool significantly improved mapping of impacted devices for five major past incidents. Many additional vulnerable devices (frequently order of magnitude higher) were found and in small fraction of time it took original vulnerability discoverers (even if they were very well familiar with CC certificates).   
%     \item Continuously updated web presentation.
% \end{itemize}


% ORIGINAL

% Tens of thousands of artifacts from Common Criteria certification framework convey detailed information about certified products. We automatically processed them, extracted inter-certificate references along with many other features, used unsupervised learning to pair the certified products with vulnerabilities in the NVD database, and performed a system-wide analysis using our newly developed open-source tool. The stakeholders can easily access our results on \url{seccerts.org} and leverage them in many ways:

% \textbf{Certificates.} Users can browse through CC and FIPS 140 certificates and see the extracted data in a concise and visually rich way. Local copies of the certification artifacts in PDF, as well as textual forms, are also accessible. The certificate page also renders an interactive graph of references.

% % In the full-text case highlighted text snippets containing the matches are also displayed.
% \textbf{Search and filtering.} The site provides both title-based and full-text searches of the certification artifacts. Such a search functionality is a powerful tool for impact assessment of vulnerabilities, as demonstrated in Section~\ref{sec:helping-vuln-research}.

% \textbf{Data.} The machine-readable data extracted using our methodology can be downloaded from the site. Our Python framework also integrates this download mechanism so users can use up-to-date processed data for their custom analysis without needing to run the data-extraction pipeline.

% \textbf{Notifications.} Users can subscribe to get email updates
% when the data associated with a certificate changes. This way, a user can be notified of new vulnerabilities that may affect certificates of their interest. These independent notifications form an additional source from where users may learn about possible problems, especially when the vendor or distributor fails to inform them. 

% \textbf{Crowd-sourcing and feedback.} Finally, we leverage the users of our site to crowd-source feedback on where our automated techniques and heuristics are wrong or where we may be missing some useful data.

% While CC certification primarily focuses on the evaluation of security claims, we demonstrated that it also impacts the security of the product. Our data reveals that acquiring higher EALs and SARs is associated with fewer and less severe vulnerabilities during the certificates' lifetime. We further identified specific SARs with the most positive impact -- providing performance evaluation crucial for designing novel lightweight certification schemes.

% %The referencing habits of certificates highlighted different usage patterns. We reported that the majority of certificates reference no other certificate. The Europe-issued certificates typically reference other Europe-issued devices (especially German-issued ones), generally due to the certification of composite products. On the contrary, US-issued certificates rarely reference any other product. 

% %Finally, as both CC and FIPS 140 certification schemes have been in use for over two decades, our tool provides useful insight into any defined temporal characteristics extracted from the certificates. We observed that the average EAL increases in time for the ICs and Smart Cards category, whereas other products exhibit stable assurance levels. In conformance with CCRA policy, we confirm that the mean certificate validity period stabilized at 5 years, despite the non-trivial number of certificates with a blank expiry date for an unclear reason. We also measured the popularity of the individual national schemes, with Netherlands and Norway gaining momentum in recent years. Last but not least, we monitor employed cryptographic primitives, seeing almost no cases of post-quantum cryptography and only slow phase-out from insecure MD5 and SHA-1 hash functions.

% Our dataset and processing framework open new possible research directions. They can be used to manually dissect peculiar certificates that may be possibly insecure. Additionally, an NLP layer to our tool could be developed to help us understand the nature of the inter-certificate references and to automate the search for misconfigured products based on the artifacts' contents. 
% Moreover, we plan to improve our framework by adding information about metadata coming from the national schemes' websites. It would also be valuable to understand the nature of the connection between CC and EMVCo~\cite{emvco} that also offers some artifacts to study. 

% %Based on the lessons learned by processing of certificates since 1997, we identified multiple issues and created list of recommendations how to improve newly issued certificates.

% % The automatic processing is issued certificates was not an easy task, as documents are written by humans primarily for other humans with many issues hindering automatic processing and decreasing usefulness of whole certification process. We propose set of recommendations to improve automatic processability, especially to increase vulnerability notification. 


% %To provide timely notification of a vulnerability found and corresponding fix, end-users typically rely on information either from the vendor or public sources like vulnerability databases. The failed notification of the Estonian government about critical ROCA cryptographic vulnerability \cite{roca} in underlying cryptographic chip impacting their eID citizen electronic document just prior to the elections is an example of notable notification failure of composite, security-certified and high-profile product.

% % To build a reference graph among the products certified under the CC and FIPS 140 certification schemes, we automatically analyzed all publicly available certification artifacts for references and other security-relevant properties. We additionally trained the classifier to pair certified products with the corresponding entries in the CVE vulnerability database with XX\% accuracy. The resulting dataset allows for automatic identification of potentially impacted composite products for every existing (and future) vulnerability using simple graph traversing. 
% % add analysis of reference type

% %Using five high-profile past vulnerabilities as the use-cases, we demonstrate that the approach is capable to quickly identify all the impacted certificates and proactively search for a set of certificates that may affect a composite product in the future. 




% % Our open-source toolchain, results continuously updated with newly issued certificates and vulnerability notifications are available for product' end-users and security researchers at \url{seccerts.org}. 




==> intro.tex <==
\section{Introduction}
Security certification frameworks such as Common Criteria (CC) \cite{cc}, FIPS 140 \cite{fips-140-2}, or EMVCo \cite{emvco} were introduced to independently evaluate the security of products and to provide increased assurance about security-relevant claims for the products' users. The frameworks offer multiple certification levels (e.g., Evaluation Assurance Levels for CC) with increasing requirements and corresponding scrutiny undertaken to verify the claims made about the product. Such evaluation comes at a non-trivial cost, both in time to obtain a certificate (months or even years) and in the required finances (hundreds of thousands of dollars or more) \cite{cost_cc,cc_overview_2017}.

Almost immediately after the CC scheme's deployment around the year 2000 (and similarly for the other schemes), discussion about its 
efficacy and limitations started and continues until today~\cite{hearn_does_2004,razzazi_common_2006,kaluvuri_quantitative_2014,swcertinpractice_2017}. The main aspects questioned are
\emph{(i)} the inadequate trade-off between the financial or time demands of the certification and the resulting assurance,
\emph{(ii)} difficult orientation of the end users in the ecosystem,
\emph{(iii)} certification being valid only for a fixed product configuration, and 
\emph{(iv)} an unfair position of the vendors with insufficient resources for the certification. Furthermore, critical vulnerabilities \cite{roca,minerva,titan,tpmfail} have been discovered in certified products with high assurance levels, which questions the very purpose of the certification. Worse, assessing their impact on issued certificates and certified products is arduous, due to the large amount of unstructured certification-related data and unclear relationships between certificates.

%Is it really that higher assurance levels associate with fewer and less severe vulnerabilities in the certified products? And what aspects of the certification have the most positive impact?

Existing research on security certifications targets, mostly qualitatively, specific products or a domain \cite{DBLP:conf/ccs/CohneyGH18}, presents anecdotal evidence about the procedural efficiency \cite{swcertinpractice_2017}, or performs a limited quantitative analysis (e.g., only EAL4+ products in \cite{kaluvuri_quantitative_2014}). A systematic insight into the whole certification practice and the security of certified products is missing. Worse, no 
%current 
research 
work studies the references between the certified products (i.e., composite or updated product) and their effect on vulnerability impact. %We speculate that this void has two main causes: \emph{(i)} limited availability of public machine-readable data from the certification processes, and \emph{(ii)} the overall complexity of measuring the product's security.

%A multitude of factors shape software/hardware security, including adherence to best security practices, security review, or extent of product testing. As a proxy measure of security, the number and severity of products' vulnerabilities are common in security research. Such a measure, however, relies on a robust mapping between the vulnerabilities and the affected products. 

%In our paper, we leverage the NVD database and map the CC-certified products to their CPE records. Together with studying the references between certified products, this enables us to compute and evaluate the number, severity, and impact of the vulnerabilities affecting  certified devices. Such analysis is possible only after overcoming numerous problems with the availability and consistency of the input data and various errors introduced by human labor during the certification process. In this work, we automatically assess all CC certificates and their artifacts to deliver the following contributions: 

In this work, we address this gap by automatically assessing all Common Criteria certificates and their artifacts to deliver the following contributions:

\begin{itemize}[noitemsep]
    \item An open-source framework for automated collection and feature extraction of security-relevant information from CC and FIPS 140 certification artifacts. Using our tool, we acquire weekly snapshots of CC and FIPS 140 certificates.
    \item An unsupervised method for mapping vulnerabilities from the National Vulnerability Database (NVD) to affected certified products.
    \item A quantitative analysis of the vulnerabilities impacting CC-certified products, driven by the mapping of  certificates to NVD.
    \item An unsupervised method for learning the inter-certificate references in all CC certificates. The resulting reference graph provides means for vulnerability impact assessment and timely notifications to the stakeholders.
    \item Multiple case studies of how our framework can be leveraged to reveal the true impact of vulnerabilities found in certified products.
\end{itemize}

%Atop of NVD vulnerability database not being complete and always accurate, the following main 
%1. Certified device not mapped to CPE
%3. CPE not corresponding to boundaries of certified configuration (ToE)
%, a reliable and complete mapping between certified products and vulnerability records in other sources like the NVD vulnerability database is not available, making it difficult to establish which of the publicly disclosed vulnerabilities are relevant to a particular certified product. 

%For example, the ROCA vulnerability (CVE-2017-15361) \cite{roca} in RSA keypair generation directly affects more than a hundred CC certificates. It is listed in the NVD database as a vulnerability in the firmware of Trusted Platform Module with 130 affected platform configurations (CPEs, mostly desktops and laptops), but none of the configurations match the affected certified items. Yet, we show that many more certified devices are, in fact, affected.

%A reliable mapping between certified product and CPE record may provide timely notification of end-users about a new vulnerability found. A corresponding fix typically relies on a vendor or public sources like vulnerability databases. Such notifications may fail even for highly sensitive and certified devices, as demonstrated, e.g., by that of the Estonian government about critical ROCA cryptographic vulnerability in their citizen eID\cite{roca}. and the possibility to proactively identify a set of certificates that may affect a composite product in the future. 

%In this paper, we answer the following research questions:

% \noindent
% \textbf{RQ1}: Can certified products be automatically mapped to records in the CVE vulnerability database?

% \noindent
% \textbf{RQ2}: What is the practical impact of increased security assurance levels on the expected number and severity of the product's vulnerabilities? 

% \noindent
% \textbf{RQ3}: How do certified products reference and affect each other?

%The open-source toolchain \texttt{sec-certs} for analysis of \textit{sec}urity \textit{cert}ificates, datasets, vulnerability notifications, and all results nightly updated with newly issued certificates are available at \url{seccerts.org}. The tool can serve many actors of the certification ecosystem: end users of the certified products, vendors, schemes administrators, or security researchers.

The paper is organized as follows: Brief introduction to Common Criteria procedures and available artifacts is given in Section~\ref{sec:background} with related work discussed in Section~\ref{sec:related_work}.
Our methodology is described in Section~\ref{sec:methodology}. In Section~\ref{sec:security_impact} we analyze the security impact of various aspects of certification. Section~\ref{sec:helping-vuln-research} presents case studies from real vulnerabilities. We discuss the 
%implications of our work and offer 
recommendations to improve certification frameworks in Section~\ref{sec:recomm}. 
%Section~\ref{sec:discussion}. 
Finally, we conclude the paper in Section~\ref{sec:conclusions}.

%Our dataset is further qualitatively evaluated using five high-profile past vulnerabilities -- demonstrating the ability to quickly identify the impacted certificates (including previously omitted cases like Estonia's eID) and the possibility to proactively identify a set of certificates that may affect a composite product in the future. 

% The schemes like Common Criteria While already in use since for more than two decades, 

% Despite such effort, serious security vulnerabilities were discovered later in the products certified even to high levels~\cite{alendal_chip_2021,roca, minerva,tpmfail,titan}, showing a gap between the intended and actual security. Due to the significant certification costs, any vulnerabilities missed by the certification process tend to persist for a number of years as the vendor is less motivated to make changes in the product which would require re-certification -- contributing to increased impact on end-users. Finally, notification of the users about a vulnerability found is typically left up to the vendor of the certified product. This is unnecessary as the product is quite precisely specified and identified (including its components, if being composite) during the certification process (e.g., Target of Evaluation in Security Target documents in CC). Automated notification would be possible if the certificate and referenced parts are uniquely identified and if such labeling is consistently used also in the vulnerability databases -- unfortunately, no such complete mapping exists today. This paper provides such a mapping and performs the related analysis.

% Additionally, a simple question like \emph{Does certification improve the security of an actual product, and is it correlated to the certification level?} seems to be difficult to answer judging on the lack of such public figures -- partially due to the complex task of measuring security in general, but also due to the burdensome to process, insufficient or missing input data for such analysis. But without the understanding of the certification efficiency, the certification procedure may become a burden preventing innovation from smaller companies due to its high cost rather than security improvement, and the well-meant improvements are ad-hoc rather than data-based. 

% Previous works unveiling the real situation of certification schemes were based on individual studies (e.g., products affected by specific vulnerability) \cite{xyz}, manual analysis on a small fraction of certificates \cite{kaluvuri_quantitative_2014} or qualitative analysis of the actual standards \cite{x,y,z}. We instead focus on the extraction of analytical information directly from public documents of all the certified products and their correlation with other relevant sources of information like vulnerability databases.

% %, automatically process them using manually labeled datasets, and pair with the other relevant sources of information like vulnerability databases. 

% We leverage the resulting processed dataset to provide insight into the state of the ecosystem, starting from general trends in the certification that runs for more than two decades, over empirical evidence of the security improvement achieved (when measured by the number and severity of the vulnerabilities found) to providing tools for vulnerability impact assessment and early notification of the product end-users.

%While CC certification is primarily focused on the evaluation of security claims, it shall also improve the practical product's security. By correlating the achieved security assurance levels with severity and time of past vulnerabilities, we identify that some security assurance requirements of the certificate are strong predictors for the expected number and the severity of the vulnerabilities the certificate is likely to suffer from in the future. Among others, \texttt{AVA\_VAN} (vulnerability analysis) and \texttt{ALC\_TAT} (tools and techniques) have the largest negative correlation with the number and severity of the expected vulnerabilities. 


==> methodology.tex <==
\section{Methodology} \label{sec:methodology}

In this section, we describe the methodology of our work, starting with a high-level description of our framework that is depicted in Figure~\ref{fig:methodology:framework}. To explore the landscape of CC-certified products, we collect, dissect and analyze the certification artifacts in the form of varyingly structured PDF documents and accompanying metadata. We begin by crawling the CC website (\numcircledtikz{1}), from which we extract links to certification artifacts along with various metadata. Next, we download (\numcircledtikz{2}) the PDF documents and convert them to text (\numcircledtikz{3}). When converted, we extract features from the text using regular expressions (\numcircledtikz{4}). Together with extracted metadata, we feed the extracted attributes into unsupervised learning models (\numcircledtikz{5}) to learn references between certificates and to link the certified products with the NVD. Finally, we evaluate these models, analyze the collected statistics and present the results to stakeholders on our web (\numcircledtikz{6}).

We release an open-source framework
\footnote{\ifanon{Code: \url{https://anonymous.4open.science/r/sec-certs-7A92}, web: \url{https://seccerts.org}}{Code: \url{https://github.com/crocs-muni/sec-certs}, web: \url{https://seccerts.org}}}
that implements all of these components. It is written in Python and also contains code for analysis of FIPS 140-2/3 certificates. On our web, we publish weekly fresh snapshots of our dataset to capture newly issued certificates and monitor possible changes in the artifacts. Our web offers an easy way to interact with our results and we envision it as an aid in vulnerability impact assessment as described later in Section~\ref{sec:helping-vuln-research}.

In the rest of this section, we examine the individual layers in detail.

\begin{figure*}[t!]
    \captionsetup{font=footnotesize}
    \centering
    \includegraphics[width=0.9\textwidth]{system_diagram.drawio.pdf}
    \caption{A high-level overview of the \texttt{sec-certs} analysis framework.}
    \label{fig:methodology:framework}
\end{figure*}

\subsection{Metadata crawling \& PDF download} \label{subsec:metadata_crawling}

First, we scrape a list of all certificates from \url{commoncriteriaportal.org}. This list is then merged with a CSV listing of certified products obtained from the same source that enriches the available metadata. To this end, we crawled records of \numCCActiveCerts{} active and \numCCArchivedCerts{} archived certificates. 
% Despite several inconsistencies between the CSV and HTML records, we consider the obtained records to be the ground truth as they were obtained from the official CC portal. 
%Among other data, 
For each certificate we obtain URLs to the following PDF documents that we download and further disseminate: \emph{(i)} certification report, \emph{(ii)} security target, and \emph{(iii)} maintenance update(s).

\subsection{PDF conversion \& feature extraction} \label{sec:methodology:subsec:pdf_to_text_conversion}

The PDF artifacts vary in their form between vendors and schemes. To enable automated processing of the documents, we convert them from PDF to text using the \texttt{pdftotext} library~\cite{pdftotext}. Some of the documents cannot be immediately parsed by \texttt{pdftotext}. We look at several attributes (text file size, a ratio of alphanumerical characters to all, etc.) to detect malformed documents. To this date, we label \numCcOcrAttempted{} documents (out of \numCcConvertAttempts) as malformed. We repair these documents by using the \texttt{Tesseract} OCR library~\cite{smith2007overview}, succeeding in \numCcOcrSuccess{} cases. After having the artifacts converted to text, we match various regular expressions in the artifacts. Using expert knowledge, we designed \numRegularExpressions{} regular expressions to extract keywords from the certification documents. The range of captured expressions is broad, from detecting terms corresponding to certificate identifiers to expressions matching cryptographic algorithms. The high-level taxonomy of these features can be seen in Table~\ref{tab:features}. The complete list of expressions is accessible from our repository\footnote{\ifanon{\url{https://anonymous.4open.science/r/sec-certs-7A92/src/sec_certs/rules.yaml}}{\url{https://github.com/crocs-muni/sec-certs/blob/main/src/sec_certs/rules.yaml}}}. The regular expressions involved in the algorithms described in the following subsections 



\begin{table}[ht]
    \centering
    \begin{tabular}{llrl}
    \toprule
    \textbf{Source}                                                & \textbf{Feature class}           & \textbf{\#}    & \textbf{Example}    \\ \midrule
    \makecell[l]{CC portal\\ (CSV,HTML)}                           & Cert. metadata                 & 14    & Vendor   \\ \midrule %14 features (form CSV and HTML)
    \multirow{2}{*}{\makecell[l]{Artifacts\\(PDF)}}                & File metadata                 & 30   & PDF Title\\ % 4 (size, enc, pagenum, links) + 11 PDF doc info = 15 (per artifact, so 30)
                                                                   & Keywords (regex)             & 64 & CC Claims\\ \midrule % 32 classes
    \multirow{4}{*}{Derivated}                                     & Certificate ID                      & 1   &                   \\
                                                                   & References                            & 8   &                 \\ % incoming and outgoing + direct and indirect + st + target and report so 2 x 2 x 2
                                                                   & CPE + CVEs                              & 2  &               \\
                                                                   & SARs                                   & 1    &               \\ \midrule
    \end{tabular}
    \caption{Overview of features extracted. Feature counts are per certificate.}
    \label{tab:features}
\end{table}

\subsection{Unsupervised learning} \label{sec:methodology:subsec:unsupervised_learning}

We use the features extracted by the previous stages of the pipeline to tackle two different problems: \emph{(i)} mapping of certified products to known vulnerabilities and \emph{(ii)} building a graph of references between certificates. We propose two unsupervised algorithms to learn the underlying problems' representations. Then, we create an expert-annotated subset of certificates to compute the precision (ratio of true positives to true positives + false positives) of the models for both problems.

\subsubsection{Mapping certified products to vulnerabilities.}

We designed a classifier that maps each certified product to a (possibly empty) list of vulnerabilities from the National Vulnerability Database that likely affects it. A prior work~\cite{kaluvuri_quantitative_2014}, manually mapped a small fraction of certificates to their CVEs. That approach, however, does not scale and cannot be automatically applied to newly discovered vulnerabilities. In contrast, our method is fully automated and works with all (also newly issued) certificates and vulnerabilities.

Every CVE in the NVD is associated with a manually crafted specification of vulnerable product configurations listed as Common Platform Enumeration (CPE) records. Given a CPE record of a product, one can traverse the NVD to find vulnerabilities that affect it. To learn what vulnerabilities affect certified products, it thus suffices to create a mapping between CPEs and Common Criteria certificates. Further in the text, we consider the mapping between CPEs and CVEs maintained by NIST as being error-free, i.e., that each CVE record contains all (but not more) CPE records that correspond to the vulnerable configurations.

CPE is a data structure consisting of fields related to a given configuration. Among others, every CPE contains the fields \texttt{<vendor>}, \texttt{<product>}, and \texttt{<version>}~\cite{waltermire_technical_2018}. To match the certified products to their CPEs, we measure the string similarity\footnote{We to measure the string similarity using a token-set-ratio and partial-ratio metrics from \texttt{RapidFuzz}~\cite{max_bachmann_2021_5584996}. } between a certificate's title and candidate CPE records. We manually fine-tuned the required similarity threshold to achieve nearly 90\% precision of the mapping on the expert-annotated samples. 

We require three conditions to hold before considering any CPE to be a candidate for a match: \emph{(i)} The CPE \texttt{<product>} field must be at least four characters long (short CPEs lead to 100\% string similarity); \emph{(ii)} vendor fields of the certificate and the CPE must match; \emph{(iii)} the major and minor versions extracted from the certificate title must match those in the CPE. For example, matching a certified product of version \texttt{5.1.2} to a CPE record with version \texttt{5.1} is allowed. This reflects the intuition that a vulnerability affecting a platform of version \texttt{5.1} also likely affects version \texttt{5.1.2}. 

% We attempted to advance our approach by matching certificate names directly to the vulnerability descriptions to bypass these problems, but this fell short of its promise, delivering deteriorated performance.
% While higher precision is possible, it asymmetrically decreases the recall, i.e., the number of matched CPE records.

\subsubsection{Building a graph of references.}
In the CC framework, every certificate (except a handful of exceptions) is assigned its own supposedly unique but structurally heterogeneous identifier (ID) under the national issuing scheme (e.g., \textit{BSI-DSZ-CC-1169-2021}). Notably, the CC framework does \emph{not} provide an authoritative pairing of certified products and IDs in public documents, nor does it provide a list of all certificate IDs, nor does it prescribe any form of these IDs. The only common characteristic of IDs across national schemes is the presence of \emph{some} counter.
Certificates often reference each other in their artifacts. The reference signals some component relationship among the certified products, such as a smartcard referencing a certificate of a cryptographic chip used within it. Such references are vital for assessing the reach of a newly found vulnerability in a certified product. For example, a vulnerability in a certified cryptographic chip may affect other certified products, such as eID cards, as witnessed during the ROCA vulnerability case~\cite{roca}. To aid this vulnerability assessment, we retrieve a full graph of inter-certificate references from the artifacts. First, we recover a unique ID to each certificate and then we search all other certificates for the presence of such ID. The ID is assigned as follows:

\begin{enumerate}[noitemsep]
    \item Extract all candidate certificate IDs using \numccschemeidrules{} regular expressions for \numccschemes{} schemes from the \emph{(i)} filename, \emph{(ii)} PDF metadata, \emph{(iii)} frontpage and \emph{(iv)} contents of the certification report of a given certificate. Assign a weight to each candidate equal to its number of occurrences.
    \item Filter candidates to match the scheme of the certificate.
    \item Canonicalize candidates, to correct errors and join variants of the same ID.
    \item Merge canonical candidates from the four sources into one list, summing the weights of duplicate candidates.
    \item Pick the candidate with the largest weight as the ID of the certificate. If there are more, pick the longest.
\end{enumerate}

\subsubsection{Model evaluation.}
\label{subsec:eval_refs_graph}
We manually verified the models' outputs on a small subset of certificates to evaluate the quality of our algorithms.

For the problem of CPE matching, we randomly sampled 100 certificates for which the model predicted at least one CPE. Two co-authors then independently annotated each of the predicted matches as true positive or false positive. The conflicting annotations were revisited by the pair of co-authors and the consensus was reached.
While this methodology does not enable us to measure the recall of our classifier, it allows for measuring its precision. That is especially relevant for CPE matching, where our results form a conservative lower bound, with probably more CPEs (and therefore vulnerabilities) applicable to the certified products. When our model declared a CPE match, it was correct in \evalCcPrecision{} cases on this expert-annotated subset. Furthermore, \evalCcRatioErrorFree{} certificates contained completely error-free matches.

For the problem of reference graph building, we manually annotated a random set of \numccideval{} certificates with their certificate IDs. This was done by one expert co-author (as there is little space for ambiguity) using the certification artifacts. We then compared the manual annotations with those assigned by our model. We observed that our classifier achieved \printpercent{\numccidevalcorrect{}}{\numccideval{}} precision. Of the cases where our model did not assign an ID (\numccmissingid{}, \printpercentfull{\numccmissingid{}}{\numcccerts{}} of the dataset) \numccmissingidunfixable{} of the errors are not fixable, mostly due to the certification artifacts containing no recognizable ID or due to the certification artifacts not being available. We also investigated certificates where our method assigned the same ID to multiple certificates, of which there were \numccduplicateid{}. Upon further analysis, \numccduplicateidcolission{} of these were due to multiple certificates sharing the same certification report files (i.e., duplicates in the input data from the CC portal).


==> recommendations.tex <==
\section{Discussion and recommendations}
\label{sec:recomm}

Based on the lessons learned through  our paper, we give recommendations that would improve the existing certification frameworks. Better, most of our recommendations require little effort to implement and, when mandated on newly certified products, would arguably improve certification transparency, vulnerability assessment, or automatic processing.




\subsection{Recommendations}

%\begin{itemize}[noitemsep]
\textbf{Assign robust certificate ID:} Unique and robust IDs assigned to each certificate allow for clear and precise referencing of related certificates. The ID shall also not be overly long to make referencing less error-prone. BSI or NSCIB formats are compact and sufficient. A format used by FIPS 140 consisting only of a counter is particularly challenging to extract unambiguously.

\textbf{Specify evaluated product boundaries more clearly:} The Target of Evaluation (ToE) is specified in a somewhat informal way, making it difficult for automatic processing to establish the ToE boundaries. Their definition is now dispersed through the certification documents, with their form prohibiting clear understanding from the stakeholders. The software equivalent of the Bill of Material (BOM) was proposed as a partial solution, but the task is more complicated: ToE covers not only the parts of the certified product but also the circumstances and environment of use. Fuzzy boundaries make it difficult for end users to verify whether the product used is in the certified configuration or to properly pair and evaluate the vulnerabilities reported. Some vendors already supply an automated tool checking if a product is running in a certified configuration. Further, while the evaluation labs act as trusted mediators to evaluate certification claims, the steps taken, tools used, and results obtained by evaluation labs are frequently confidential and not independently replicable later. At least part of the tests shall be automated and made with product results openly available. 

\textbf{Pre-assign platform records (e.g., CPE) to certificates:} Well-defined records remove ambiguity in certificate naming and enable more accurate assignment of vulnerabilities to the affected platform(s), resulting in a complete bidirectional linking between certified products and %a database of
vulnerabilities. Some products, like operating systems, consist of multiple software packages or other components. As the certification procedure already requires the vendor to monitor a vulnerability database for relevant vulnerabilities, the vendor likely has a list of CPEs to watch that could be made public.

\textbf{Define and use pre-defined machine-readable templates}. As the certified products from the same category and/or implementing the same Protection Profile frequently follow a very similar structure, pre-defined templates would not only speed up document preparation but, more importantly, also allow for automated checks against predefined criteria and options selected. Not surprisingly, such templates are already in use, as one can say from the documents prepared by some of the larger vendors, but are not publicly available and cross-compatible.  

% \textbf{Create a component structure for composite products:} We demonstrated that the density of inter-certificate references is relatively low. Thus, documentation of referenced components along with their type (e.g., using Security Content Automation Protocol~\cite{waltermire_technical_2018}) should be possible.

\textbf{Be more transparent in vulnerability handling:} While the certified products can include patches that protect them from existing vulnerabilities that otherwise affect the product of such a version, the information about whether these patches are applied is not transparent. Maintenance updates often neglect vulnerabilities or present generic statements like \emph{\enquote{IAR contains a rationale why these vulnerabilities do not affect the ToE}}. We recommend that IARs get disclosed as a part of the maintenance and that all vulnerabilities considered during the maintenance are explicitly listed with their IDs. Additionally, the IAR should clearly comment on the rationale for considering some vulnerabilities as out-of-scope.

\textbf{Provide a clear reason for certified product validity end:} A reason for a product archival helps end-users to assess its further usage, especially for a product with non-standard or a prematurely ending validity period (e.g., due to unfixable vulnerability or a mistake in certificate issuance). The certification scheme acts here as an independent and trusted party, since the product vendor might be in a conflict of interest to fully and timely disseminate the reason for certificate validity termination. The inspiration can be taken from handling and revoking web PKI certificates, possibly including automated validity check services like Online Certificate Status Protocol (OCSP).  

%    \item \emph{Enforce unified document formatting} of the certification documents, preferably in English. From some of the certificates, text cannot be easily extracted for subsequent analysis. 

\textbf{Design certification tests for replicability:} Evaluation labs function as trusted mediators that allow the assessment of certification claims based on proprietary (non-public) documents. But steps taken, tools used, and results obtained by evaluation labs are frequently confidential. Moreover, the level of expertise found in specialized evaluation laboratories is not available to all end users. Public documents, like maintenance reports, also frequently lack the data used during their issuance. As a result, certification and subsequent annual re-evaluations of a product are usually done by the same lab. Due to confidentiality, these activities are not independently replicable later. Test automation and detailed description of the steps taken, preferably with openly available tools, would allow for better replicability and retrospective assessment.% (was my product tested against a particular attack?). 

\textbf{Improve data quality served by official certification portals:} The primary sources of certification artifacts \cite{cc_webpage,fips_webpage} contains inaccuracies like improperly formatted CSV files with duplicate rows, non-existent links, missing or incorrect valid until date, duplicated documents, or corrupted files. 

\textbf{Make information available in standardized, machine-readable formats:} Cost of creation of an additional metadata file is likely negligible with respect to overall certification cost but significantly improves the usefulness of certification artifacts after the certification is finished.

\subsection{Limitations}
\label{sec:limitations}

Our analysis has several limitations, mostly due to incomplete or inconsistent input data. We discuss their possible impact on the presented results below.

\noindent \textbf{Noisy data.} The certification documents are a free-form, often ambiguous, and inconsistent data source. We mitigate some errors by augmenting inputs (e.g., CC product lists from both CSV and HTML inputs). Where possible, we measure the precision of our heuristics on manually annotated certificate subsets.

%\textbf{Only public data is processed:} During certification, additional artifacts are created that remain confidential between the vendor, evaluation facility, or certification scheme. Our analysis would benefit from the features embodied therein. The ability to harvest these could lead to a richer graph of references or to more reliable vulnerability matching.

\noindent \textbf{Unclear ToE boundaries.} A security target specifies the boundaries of the evaluated product, which typically do not span all product components. Yet, our mapping of certificates to vulnerabilities cannot account for a limited ToE and considers all parts of a product to be inside the ToE. While technically an error, we believe that this generally matches the expectations of end-users. 
The unclear boundary is even more pressing given anecdotal evidence that vendors may purposely limit the ToE scope in order to limit the attack surface during the evaluation instead of improving the security of the product and fixing potential vulnerabilities.
As an example of such issue, consider the certificate~\cite{sertit-115} of a \emph{network} camera. Its network interface was considered to be always trusted and therefore likely untested during its evaluation.\footnote{The certification report~\cite{sertit-115} states: \enquote{Attackers have no chance to connect any malicious devices into the local network of the TOE.}} 

\noindent \textbf{Limitations of NVD.} Not all vulnerabilities are assigned a CVE record and/or adequately equipped with affected platform CPEs. Here, our work forms a lower bound on the number of vulnerabilities in certified products with more likely existing. 

\textbf{Context-free references:} While many certificates reference others to signal a sub-component relationship, this may not always be the case. As our reference analysis does not distinguish the reference context, false positives are possible when using the graph of references for assessment of vulnerability impact. To measure the scope of this issue, we performed a manual analysis of references in \numCcRefEval{} certificates that we reported in Subsection~\ref{subsec:eval_refs_graph}.











==> relatedwork.tex <==
\section{Related Work}
\label{sec:related_work}

We divide the studied papers into three different categories: \emph{(i)} papers that identify problems in certification schemes, often suggesting improvements; \emph{(ii)} papers that try to make sense of the certification process, often case-study driven; \emph{(iii)} more recent papers that work towards automated processing of security-related documents, possibly leading to automated and transparent certification.  
Most of the research on CC and FIPS 140 certification schemes builds on individual case studies, which also limits the range of results, as the authors are mostly steered by intuition, not backed with large-scale data analysis. An exception is a study~\cite{kaluvuri_quantitative_2014} that exploits data-driven analysis of CC scheme, parsing metadata from its website. The study, however, focuses only on a subset of certificates, omits the analysis of the certification-process-related documents, and resorts to manual labor when examining vulnerabilities. Being limited only to EAL4+ certificates forming only around 40\% of the dataset at the time of the paper writing, the results are relevant only for the domain of ICs and smartcards, which differs significantly from the other categories as demonstrated by our analysis.

%\subsection{Problems of certification}
In~\cite{hearn_does_2004}, Hearn expresses the challenges that the CC faced around 2004. Eight years later, Murdoch et al.~\cite{murdoch_how_2012} discuss why both CC and FIPS 140 fail short of their promise, pointing to the lack of transparency, a problem that still prevails. More of a political perspective is taken in~\cite{kallberg_common_2012} that describes the fragility of international standards relying on national alliances that may not last forever. Beckert et al.~\cite{Beckert2010MindTG} studies the intriguing fact that CC requires formal verification of the specification to achieve high EALs. Still, the implementation is not formally verified, despite the recent advances in the field. Many of the schemes' problems articulated in our work are also mentioned in a user study~\cite{haney_organizational_2018} of 29 users trained in NIST cryptographic standards and validation programs.%\todo{Lukasz, two things to discuss: (1) present vs. past tense (2) citation style (sentence with citation removed point). For me all is fine as I am not a native speaker (just want to raise it). }

%\subsection{Understanding certification}
To many, CC and FIPS 140 appear so complex and opaque that it is difficult to understand how one can obtain a certificate and what implications the certification has. This is tackled by several papers that explain the certification process or provide guidance on how to approach it~\cite{cc_overview_2017,mellado_common_2007,herrmann_using_2003,razzazi_common_2006,vetterling_secure_2002,kacprzyk_patterns_2011}. Some works focus on individual product domains for which they provide support (e.g., IoT devices)~\cite{rogowski_2014,bialas_common_2010,kaluvuri_bringing_2013,kang_how_2017}. An interesting study~\cite{shapiro_understanding_2003} dissects the CC-certified (EAL4) Windows version from 2004 and demonstrates the limited practical meaning of EAL levels without considering actual evaluated usage scenario (non-hostile and well-managed user community in this case). A recent paper from 2019 studies the costs introduced by securing software, targeting CC as well~\cite{venson_costing_2019}.

%\subsection{Automated processing of documents}

We believe that much precious information is hidden in the PDF artifacts of security certifications. Recent advances in the area of Natural Language Processing (NLP) could be leveraged to translate therein achieved results into the world of information security. This was already suggested for FIPS 140 
%documents 
by Vassilev~\cite{vassilev2019bowtie}, and performed for the privacy-policies domain by Harkous et al.~\cite{polisis}. Similarly, a study from 2014~\cite{riaz_hidden_2014} attempts to automatically identify security-related sentences and security requirements from natural language artifacts using machine learning. Translating these results into the area of security certificates could allow for automated analysis of potentially vulnerable configurations. In~\cite{DBLP:conf/ccs/CohneyGH18}, Cohney et al. demonstrated that manual analysis of FIPS 140 security policy documents can yield discoveries of critically flawed PRNG configurations.

In our work, we relied on the mapping between CVEs and the associated CPEs as provided by the NVD. But even constructing such mapping solicits active research. The respective papers try to make this process more efficient and complete, or less erroneous~\cite{tovarnak_graph_2021,wareus_automated_2020,sanguino_software_2017}.

A closed-source tool called \emph{CCScraper}~\cite{ccscraper-2021} %\footnote{The tool is annually used to present a statistical analysis of the CC landscape at the International CC Conference, \url{https://iccconference.org/}. The last available presentation was given in 2021, see \url{https://www.jtsec.es/papers/CC/ICCC21\%202021\%20Statistics\%20Report.pdf}.}
developed by the jtsec security lab in 2018 automatically analyzes information from the CC and Certification Scheme portals using OCR capabilities and other features. While the tool seems similar to our \texttt{sec-certs}, there are notable differences -- it is not oriented at certification process evaluation using the NVD database, and it does not seem to produce a graph of references usable for vulnerability notification. As the tool is not publicly available, we cannot provide a more detailed comparison. 
%On the other hand CC scraper merges the certificate metadata from the national schemes' websites into the database while we keep that data separate. Unfortunately, due to CC scraper being closed-source, we were not able to compare it to \texttt{sec-certs}. 

In contrast to prior work, we fully automate the analysis of certification artifacts. Better, we learn the references between the certificates and map the certified products to existing vulnerabilities, quantitatively exploring the association between the level of certification requirements and severity of vulnerabilities found on all items certified under Common Criteria. 


==> security_impact.tex <==
\section{Measuring security impact of certification} \label{sec:security_impact}

In this section, we apply the classifier described in Section~\ref{sec:methodology} that maps certificates to vulnerabilities to examine relations between vulnerabilities and the certified products. With our analysis, we aim to answer several intriguing questions: When, in the life-cycle of the certified product do the vulnerabilities tend to appear? What are the most common weaknesses that affect certified products? Does the distribution of the weaknesses differ between open-source projects and certified products? What is the role of the maintenance updates (a formal step in certification process) in vulnerability remediation? And finally, is number and severity of the vulnerabilities associated with the degree of scrutiny that a product undergoes during the certification process? 

Before we answer these questions, we first assess our data resource, the National Vulnerability Database. NVD is arguably the most widely used database of vulnerabilities. Better, it is manually curated and vetted. As such, NVD has proven a central resource for assessing vulnerability impact and remediation in various ecosystems~\cite{security-patches,security-vulns-python}, and its data backs many security tools\footnote{Such security tools include: Lacework, Snyk, Veracode, or others.}. Still, it must be understood that a small fraction of records may exhibit inconsistencies~\cite{cleaning-nvd} and that not all exploitable vulnerabilities may get their CVE issued. During our investigation, we noticed that this is the case, especially for the smartcard industry that does not consider the CVE database as the primary means for vulnerability reporting\footnote{Search for various forms of \enquote{smartcard} in NVD returns only handful of results.}. In our dataset, we register a major discrepancy between the number of certified smartcards and a number of certified smartcards with a vulnerability. In fact, we detected only \numSmartcardsDistinctVulnerabilities{} distinct vulnerabilities for this category with \numSmartcardsVulnerable{} vulnerable certificates in total. \numSmartcardsRocaVuln{} certified smart cards suffer from the ROCA~\cite{roca} and \numSmartcardsTitanVuln{} from Titan~\cite{titan_cve} vulnerability, both high-profile flaws. For that reason, smartcards are further omitted from the rest of this section. We affirm that the ratio of CVE-rich certified products to all certified products is uniform in \emph{all other categories}.

\begin{table}[b]
\scalebox{0.7}{
\begin{minipage}[b]{0.7\linewidth}
\centering
\begin{tabular}{ c | c | c }
\toprule
\textbf{CWE-ID} & \textbf{CWE name} & \textbf{\# CVEs} \\
\midrule
CWE-119	 & Buffer overflow 	 & 892 \\
CWE-20	 & Improper Input Validation 	 & 487 \\
CWE-200	 & Sensitive information exposure 	 & 349 \\
CWE-264	 & Access control error 	 & 316 \\
CWE-787	 & Out-of-bounds Write 	 & 297 \\
CWE-125	 & Out-of-bounds Read 	 & 208 \\
CWE-399	 & Resource Management Errors 	 & 180 \\
CWE-79	 & Cross-site Scripting 	 & 148 \\
CWE-416	 & Use After Free 	 & 122 \\
CWE-362	 & Race Condition 	 & 115 \\
\bottomrule
\end{tabular}
\vspace{2mm}
\caption{Top 10 weaknesses (CWEs) identified from 3114 vulnerabilities that affect 362 distinct CC-certified products.}
\label{tab:cwes}
\end{minipage}\hfill
\hspace{0.2cm}
\begin{minipage}[b]{0.68\linewidth}
%\centering

\input{cve_hist.pgf}
\captionof{figure}{Disclosure dates of CVEs that affect certified products in relation to the certification date.}
\label{fig:vuln_histogram}
\end{minipage}
}
\end{table}


\subsection{Vulnerabilities in certified products}

Among \numCCActiveCerts{} active (\numCCArchivedCerts{} archived) certificates, we identified \numCCActiveVulnerable{} (\numCCArchivedVulnerable) with at least one assigned vulnerability. As can be seen from Figure~\ref{fig:vuln_histogram}, approximately \numVulnerableCertsBeforeCertification{} of vulnerabilities were publicly disclosed in the NVD \emph{before} the certification date. This means that the majority (\numVulnerableCertsAfterCertification{}) of vulnerabilities were disclosed after the security evaluation related to CC certification process. Worse, if a certified product got affected by a CVE, in \numVulnerableCertsInValidityPeriod{} cases it was during its certificate's lifetime. In the rest of this section, we study only the vulnerabilities disclosed during the validity period of the product.

We also investigated certificates with a validity period shorter than 365 days. While it is not transparent whether a certificate was withdrawn or set to expire that soon (this information cannot be publicly backtracked), it is highly unlikely that a certificate would be intended to be valid for less than a year. In our data, we identified \numCertsRevokedWithinYear{} such certificates. Yet, we register a CVE only for \numVulnerableCertsRevokedWithinYear{} of them. We, therefore, conjecture that the vendors revoke the certificates early for reasons mostly unrelated to \emph{publicly} disclosed vulnerabilities.

\subsection{Most common weaknesses}

Many of the vulnerabilities in the NVD are manually assigned a set of so-called common weaknesses from the Common Weakness Enumeration (CWE)~\cite{cwe} that capture the cause and nature of the vulnerability. We linked the vulnerabilities occurring in CC certificates to their weaknesses, learning what weaknesses cause most harm in the landscape of certified products%\footnote{While the taxonomy of CWEs is a forest-like structure with different levels of abstraction, NVD uses only a subset of those in its CVEs.}
. Table~\ref{tab:cwes} shows a diverse set of weaknesses affecting certified products with buffer overflow, improper input validation, and sensitive information exposure being the most common. The prevalence of weaknesses in our dataset does not change dramatically over time and the distribution is comparable to the one reported in the landscape of open-source projects by Bhandari et al.~\cite{bhandari2021cvefixes} (all their top-8 CWEs are present in our top-15 list). This experiment shows that the certified products suffer from weaknesses similar to those identified in the open-source projects.


\subsection{Higher EAL, fewer vulnerabilities?}

The CC standard categorizes~\cite{cc_sars_2017} Security Assurance Requirements into multiple classes that convey different aspects of product security. For instance, the \texttt{ATE} class stands for \textit{tests}, whereas the \texttt{AVA} class stands for \textit{vulnerability assessment}. The classes are further split into families. For example, \texttt{ATE\_COV} specifies test coverage while \texttt{ATE\_DPT} specifies test depth. Each of these families has a different domain of levels with free-text descriptions. For example, \texttt{ATE\_COV} can be of levels 1, 2, or 3, depending on the test coverage during the development. These fine-grained requirements are the basis for more coarse EALs.


\begin{table*}[t]
\captionsetup{font=scriptsize}
\centering
{\scriptsize
\begin{tabular}{ c | c c | c c | c c }
    \toprule
    & \multicolumn{2}{ c |}{\emph{number of CVEs}} &  \multicolumn{2}{ c |}{\emph{Average CVE base score}} & \multicolumn{2}{ c }{\emph{variable characteristics}} \\
    variable & $\rho$ & p-value & $\rho$ & p-value & support & domain range \\
    \midrule
EAL &  -0.02 &  1.64e-01 & \cellcolor{green!15} -0.28 & \cellcolor{green!15} 4.24e-05 & 2927 & 14 \\
ALC\_CMS & \cellcolor{green!15} -0.07 & \cellcolor{green!15} 7.34e-05 & \cellcolor{green!15} -0.35 & \cellcolor{green!15} 2.55e-07 & 2583 & 5 \\
ALC\_CMC & \cellcolor{green!15} -0.08 & \cellcolor{green!15} 3.54e-05 & \cellcolor{green!15} -0.35 & \cellcolor{green!15} 3.05e-07 & 2578 & 5 \\
AVA\_VAN & \cellcolor{green!15} -0.08 & \cellcolor{green!15} 1.29e-05 & \cellcolor{green!15} -0.34 & \cellcolor{green!15} 6.47e-07 & 2606 & 4 \\
ATE\_COV &  -0.03 &  8.50e-02 & \cellcolor{green!15} -0.33 & \cellcolor{green!15} 8.41e-06 & 2419 & 3 \\
ATE\_IND & \cellcolor{green!15} -0.05 & \cellcolor{green!15} 1.51e-03 & \cellcolor{green!15} -0.29 & \cellcolor{green!15} 1.54e-06 & 3321 & 3 \\
ADV\_FSP & \cellcolor{green!15} -0.06 & \cellcolor{green!15} 4.19e-04 & \cellcolor{green!15} -0.24 & \cellcolor{green!15} 6.00e-05 & 3371 & 6 \\
ASE\_OBJ & \cellcolor{green!15} -0.07 & \cellcolor{green!15} 1.33e-03 &  -0.14 &  4.46e-02 & 2080 & 2 \\
ASE\_REQ & \cellcolor{green!15} -0.07 & \cellcolor{green!15} 2.94e-04 &  -0.12 &  6.01e-02 & 2120 & 2 \\
ALC\_FLR &  0.06 &  9.94e-01 &  0.14 &  9.52e-01 & 1684 & 3 \\
    \bottomrule
\end{tabular}
}
\vspace*{0.5em}
\caption{Spearman's rank correlations between SARs (EAL) and two attributes extracted from the certified product: number of CVEs and the average CVE base score. The \emph{support} column denotes the sample size for the given pair of variables. The \emph{domain range} 
%column 
displays the number of distinct ranks empirically measured in the given SAR or EAL. The p-value is associated with the null hypothesis \emph{\enquote{The examined variables are not negatively correlated}}. Associations with p-value $<0.01$ (higher SAR level likely leads to less severe vulnerabilities) are highlighted. 
%with color. 
We report 
%this as 
a full list of the examined associations during our study.}
\label{tab:correlations}
\vspace*{-1em}
\end{table*}
%\todo{Add human-readable names for SARs}


It is natural to hypothesize that products validated to higher assurance levels will suffer from fewer and less severe vulnerabilities. In other words, the levels of SARs (EAL) should be negatively associated with those variables. Using our tool, we reconstructed the SAR levels of a certificate from three sources: \emph{(i)} assurance level field in the CC-provided CSV file, \emph{(ii)} keywords in the Security Target, \emph{(iii)} keywords in the Certification Report. Based on this information, we established a set of certificates' SARs. We then measured the association between SARs (EAL) and two variables: \emph{(i)} Number of CVEs that the product suffered from \textit{during its validity period}; \emph{(ii)} Average \textit{base score} (severity) of the related vulnerabilities (from the Common Vulnerability Scoring System~\cite{cvss}). Given the ordinal nature of the variables, Spearman's rank correlation coefficient ($\rho$) was used to measure the association. To have sufficient sample sizes, we focused on SARs with $>100$ vulnerable certificates and a diverse domain\footnote{At least two SAR levels found, each in $>40$ certificates.}, which yielded an analysis of $9$ distinct SARs. All reported findings were computed on the confidence level $0.99$ using a one-sided alternative hypothesis that the variables \emph{are negatively} correlated.  

We report the following results: 7/9 SARs are negatively associated with the number of CVEs affecting the given certificate. The associations, however, are very weak, with $\left | \rho \right | \leq 0.07$. More importantly, 6/9 SARs are negatively associated with the average base score of the affecting vulnerabilities, showing a strong relationship with $0.24 \leq \left | \rho \right | \leq 0.35$. These are: functional specification, independent testing, test coverage, vulnerability assessment, configuration management capabilities, and configuration management scope. Interestingly, EAL is correlated only with the average base score of the vulnerabilities, with $\rho = - 0.28$. We did not encounter a positive association during our experiments. This experiment shows what security requirements have the highest association with lower average CVE base scores, possibly preventing catastrophic bugs. %The full table with the correlations can be found in Appendix~\ref{sec:app:correlations}.

% \begin{table}[ht]
% \scalebox{0.7}{
% \begin{minipage}[b]{0.7\linewidth}
% \centering
% \begin{tabular}{ c | c | c }
% \toprule
% \textbf{CWE-ID} & \textbf{CWE name} & \textbf{\# CVEs} \\
% \midrule
% CWE-119	 & Buffer overflow 	 & 863 \\
% CWE-200	 & Sensitive information exposure 	 & 608 \\
% CWE-20	 & Improper Input Validation 	 & 582 \\
% CWE-787	 & Out-of-bounds Write 	 & 490 \\
% CWE-269	 & Improper Privilege Management 	 & 466 \\
% CWE-264	 & Access control error 	 & 287 \\
% CWE-125	 & Out-of-bounds Read 	 & 255 \\
% CWE-362	 & Race Condition 	 & 199 \\
% CWE-399	 & Resource Management Errors 	 & 161 \\
% CWE-416	 & Use After Free 	 & 155 \\
% \bottomrule
% \end{tabular}
% \caption{Top 10 weaknesses (CWEs) found in CC certified products.}
% \label{tab:cwes}
% \end{minipage}\hfill
% \hspace{0.2cm}
% \begin{minipage}[b]{0.68\linewidth}
% %\centering

% \input{figs/cve_hist.pgf}
% \captionof{figure}{Disclosure dates of CVEs that affect certified products in relation to the certification date.}
% \label{fig:vuln_histogram}
% \end{minipage}
% }
% \end{table}


\subsection{Do maintenance update fix CVEs?}

% \begin{figure}
%     \centering
%     \input{figs/cve_hist.pgf}
%     \caption{Histogram displaying disclosure dates of CVEs that affect certified products in relation to the certification date.} %The x-axis displays days before (negative values) or after (positive) the date of certification (red line). The y-axis shows the absolute frequency of vulnerabilities disloced for the given certificates.} %As the plot suggests, majority of CVEs are disclosed \emph{after} the product is certified and large mass also well within the validity period.}
%     \label{fig:vuln_histogram}
% \end{figure}


% \begin{table}[t]
% \centering
% \begin{tabular}{ c | c | c }
% \toprule
% \textbf{CWE-ID} & \textbf{CWE name} & \textbf{\# CVEs} \\
% \midrule
% CWE-119	 & Buffer overflow 	 & 863 \\
% CWE-200	 & Sensitive information exposure 	 & 608 \\
% CWE-20	 & Improper Input Validation 	 & 582 \\
% CWE-787	 & Out-of-bounds Write 	 & 490 \\
% CWE-269	 & Improper Privilege Management 	 & 466 \\
% CWE-264	 & Access control error 	 & 287 \\
% CWE-125	 & Out-of-bounds Read 	 & 255 \\
% CWE-362	 & Race Condition 	 & 199 \\
% CWE-399	 & Resource Management Errors 	 & 161 \\
% CWE-416	 & Use After Free 	 & 155 \\
% \bottomrule
% \end{tabular}
% \caption{Top 10 weaknesses (CWEs) in CC certified products.}
% \label{tab:cwes}
% \end{table}


In CC, the vendors can participate in so-called assurance continuity~\cite{assurance_continuity} that enables making minor or major changes to the ToE without repeating the whole product evaluation. The bug fixes to ToE can be released in so-called \emph{maintenance updates} if they are categorized as minor changes. The the analysis of the bug is, however, hidden in undisclosed Impact Analysis Report (IAR). 

We searched for all certificates that exhibited at least one vulnerability \textit{after they were certified and before a maintenance update was released}, manually investigating the contents of the respective update documents to learn their rationale. This yielded \numVulnerableCertsWithMaintenance{} updates to study that all conveyed some vulnerability analysis. Three encountered scenarios were particularly troubling. First, one update contains the phrase \enquote{The guidance document has been updated to ensure a vulnerable feature, which is disabled by default, remains disabled.}. This suggests that the vulnerable feature remains in the product, and the user is instructed not to trigger it. Second, one of the products used a maintenance update (issued 3 years after certification) to fix 3 CVEs that were publicly disclosed before the product was \emph{initially} certified, showing a considerable delay. And third, multiple updates argued that the detected vulnerabilities fall out of ToE's scope, with the rationale being elaborated in IAR that is not available for public scrutiny. 

% TODO: Add a sentence of implications, scream out loud "this must be more transparent"


==> vuln_research.tex <==
 \section{Improving vulnerability mitigation} \label{sec:helping-vuln-research}
Our methodology and data improve the impact assessment of vulnerabilities discovered in certified products. There are several benefits to certification ecosystem stakeholders: end-users can get early notification of a potential vulnerability for the products they use, security researchers can shortlist candidates for further scrutiny and responsible disclosure, and vendors can assess their certified products. Importantly, end-users are not dependent solely on the information flow from the vulnerable product vendor, which may have misaligned incentives hindering timely notification or may not be able to directly contact the end-user -- as is the case when a product is sold via intermediaries.

To demonstrate the contributions of our tool, we analyze four past vulnerabilities and compare the information obtained using \texttt{sec-certs} with a mature understanding of the vulnerabilities. We cover  different types of vulnerabilities: algorithmic vulnerability in RSA keypair generation in Infineon cryptographic chips (ROCA \cite{roca}), timing-leakage vulnerabilities in STM chips and several cryptographic libraries (TPMFail \cite{tpmfail} and Minerva \cite{minerva}), and an EM-leakage vulnerability in several smartcards (A Side Journey to Titan \cite{titan}).

We note that such an evaluation is qualitative rather than quantitative. It is undoubtedly easier to search for something knowing it exists, i.e., affected products. The evaluation might be biased due to the vulnerability type (we are investigating only several high-profile vulnerabilities) or the affected product type (we focus on the domain of cryptographic hardware where we expect higher benefits due to overall ecosystem secrecy and obscurity).
%\enlargethispage{1cm}

%\subsection{Failed notification of Estonian estID} \label{subsec:case-estonia-fail}
\subsection{ROCA (CVE-2017-15361)} \label{subsec:case-roca}

To demonstrate our method, we begin with the case of Estonian eID documents utilizing a chip vulnerable to the ROCA attack \cite{roca} with certificate ID \href{https://seccerts.org/cc/350581534e265186/}{ANSSI-CC-2013/55} \cite{estIDCert}. After the responsible disclosure of the vulnerability to Infineon (the manufacturer of the vulnerable chip) by the original researchers, large affected parties were supposed to be notified before the public disclosure, either by the eID vendor or via non-public memos distributed among the parties involved in the EU-wide eIDAS directive. However, the Estonian government received the vulnerability information only at the beginning of September 2017, close to the municipal elections with e-voting utilizing the eID cards with the vulnerable chips. While we cannot assess the information distributed by the vendor directly, we can analyze the information distributed in the eIDAS incident report memo ID 163484 
%it is official name in google, I do not apply comment by Vashek
issued to all EU members on 20th of June 2017 \cite{eidasmemo} by an affected Austrian e-health provider. That memo was insufficient for the Estonian government to become aware of the impact. 

The memo states that \enquote{CardOS V5.0 with Application for QES, V1.0} and \enquote{CardOS V5.3 QES, V1.0} are vulnerable (directly corresponding to certificates \href{https://seccerts.org/cc/5ee9898421c06859/}{BSI-DSZ-CC-0833-2013} and \href{https://seccerts.org/cc/7e8763f553e43d12/}{BSI-DSZ-CC-0921-2014}). Also, a \enquote{weakness in asymmetric crypto library} was mentioned and that the \enquote{problem affects generating electronic signature creation data for use with the RSA algorithm} was noted. A concrete vendor was named in the memo, which was not the manufacturer of the vulnerable chip, but a platform integrator instead. Using these two certificates, we search for references from these certificates, which gives us two chip certificates: \href{https://seccerts.org/cc/8eb6fca41668f95b/}{BSI-DSZ-CC-0758-2012} and \href{https://seccerts.org/cc/9be76c10474e0c80/}{BSI-DSZ-CC-0782-2012}. 
Both certificates are a version of Infineon Security Controller M7892 with \enquote{optional RSA2048/4096 v1.02.013 ... libraries}, matching the weakness description from the memo. Having the vulnerable chip certificates, we can search for certificates  referencing them. More than one hundred certificates are found, yet Estonia's 
%Lukasz: to me it looks good no?
\href{https://seccerts.org/cc/350581534e265186/}{ANSSI-CC-2013/55} is not among them as it uses a different certified chip (but with the same cryptographic library). Additionally, the cluster of devices related to these named in the Austrian report is only very indirectly connected to the cluster \href{https://seccerts.org/cc/350581534e265186/}{ANSSI-CC-2013/55} belongs to. To match \href{https://seccerts.org/cc/350581534e265186/}{ANSSI-CC-2013/55}, we need to create the initial set of vulnerable certificates from all chips with the vulnerable \texttt{RSALib v1.02.013} library and build a reference graph from this set -- crucial insight that requires understanding what was shared between the two certified products in the memo, as well as the description of the weakness. Automatic search alone would not be sufficient in this case, but relatively simple refinement with input from a security expert is sufficient.

After the public disclosure of the ROCA vulnerability \cite{roca}, many end-users attempted to determine whether they were impacted. While, in this case, it was possible to detect the vulnerable product directly from the statistical properties of generated public keys, such an option is not readily available in general. The corresponding CVE-2017-15361\footnote{\url{https://nvd.nist.gov/vuln/detail/CVE-2017-15361}} description illustrates the case of incomplete or even misleading information about a specific vulnerability in NVD. While the CVE initially listed the exact version of the vulnerable library, it mentioned only TPM chips with CPEs mostly consisting of affected laptop platforms -- omitting the fact that large majority of Infineon smartcards was also vulnerable as the same library was used.

As the vulnerable library version is publicly known from the CVE description, we 
%can 
search for the strings \enquote{RSALib} and \enquote{1.02.013} using the CC portal \cite{cc_webpage}; this yields only 3 and 32 certificates, respectively. In contrast, \texttt{sec-certs} directly links \numSmartcardsRocaVuln{} certificates to the CVE. 
%to ROCA CVE. 
Additionally, we automatically find \numCertsReferencingRocaVuln{} certificates that reference the vulnerable ones, a significant improvement. %The resulting cluster is also visually inspectable in graph of references. 

%Still, additional questions remain: Is library version 1.02.013 the only vulnerable? Will my device's certificate mention usage of RSALib v1.02.013 directly or just reference other certificate with vulnerable RSALib component? Is my device actually utilizing the vulnerable functionality? 

\subsection{TPM-Fail (CVE-2019-16863)} \label{subsec:tpmfail}
The TPM-Fail paper presented a timing attack vulnerability 
%\cite{tpmfail_cve} 
\footnote{\url{https://nvd.nist.gov/vuln/detail/CVE-2019-16863}}
on ECDSA signing in several TPM implementations, including a CC and FIPS 140-2 certified chip, the \textit{ST33TPHF2ESPI} with firmware version 73.04 \cite{tpmfail}. The paper points to the \href{https://seccerts.org/cc/10b17081dd7cad8f/}{ANSSI-CC-2018/41} certificate as vulnerable. Also, it links to the product brief of the chip, which advertises CC and FIPS 140-2 certifications, but does not point to concrete certificates. Additionally, the CVE listing from NVD provides several CPEs that include the chip name in few variations and firmware versions.

Using \texttt{sec-certs}, we can search for the chip name and firmware versions, yielding 5 CC certificates, including the one mentioned in the paper. By looking at references of the found certificates, we uncover 7 additional certificates concerning the same family of \textit{ST33TPHF2*} chips. Comparing their reported firmware versions with the CPEs from NVD leads to 6 certificates matching the vulnerable versions, while the original paper reported only the one.

%Searching the FIPS 140 certificates yields 6 results. At first sight a different versioning scheme appears to be in use in these security targets (version prefix of \textit{49} instead of \textit{73}) and we find no certificate that would directly match the reported vulnerable versions. However, the CC targets do mention the possibility of version number being reported in hexadecimal, which fits in this case as \textit{0x49} is equal to \textit{73}. If we take this into account we find three certificates matching the reported vulnerable versions.

%\todo[backgroundcolor=green]{JanJ: Add note that we do not match the CVE to anything currently (sadly).}


\if0
https://nvd.nist.gov/vuln/detail/CVE-2019-16863

ST33TPHF2E
\url{https://seccerts.org/cc/ftsearch/?q=st33tphf2e&cat=abcdefghijklmop&status=any&type=any}

Search on seccerts gives:
 - https://seccerts.org/cc/01dc77d7f8f94d97/  ANSSI-CC-2019/53
 - https://seccerts.org/cc/0bd759633c0ceec6/  ANSSI-CC-2018/39
 - https://seccerts.org/cc/10b17081dd7cad8f/  ANSSI-CC-2018/41 <- mentioned in paper
 -  https://seccerts.org/cc/27baf39406deb767/  ANSSI-CC-2018/41 <- also gives same ID, likely a collision
 - https://seccerts.org/cc/3df01446a2b92093/  ANSSI-CC-2019/52 <- tool did not get ID
 - https://seccerts.org/cc/6b605ff743c859d0/  ANSSI-CC-2019/37

From looking at ref graph:
 - https://seccerts.org/cc/4b3f577896c80f8a/ ANSSI-CC-2016/77
 - https://seccerts.org/cc/a5898123ec124b34/ ANSSI-CC-2016/78
 - https://seccerts.org/cc/4f953ae00a24eb85/ ANSSI-CC-2017/39
 - https://seccerts.org/cc/22ede463dbf1a105/ ANSSI-CC-2017/40
 - https://seccerts.org/cc/4b3f577896c80f8a/ ANSSI-CC-2017/38
 

Bunch of cpe:2.3:h:st:st33tphf2espi:-:*:*:*:*:*:*:* like CPEs on the CVE.

Paper mentions: ST33TPHF2ESPI with STMicro 73.04 firmware
then lists ANSSI-CC-2018/41 as the vulnerable chip. Points to the product brief for ST33TPHF2ESPI.

FIPS seccerts search gives 6 certs, some of which are still valid.

But we do not map the CVE to any certs :(
\fi

\subsection{Minerva (CVE-2019-15809)}
The Minerva group of timing attack vulnerabilities in ECDSA signing \cite{minerva} coincided with and exploited the same type of leakage as TPM-Fail, but targeted a different set of implementations, including smartcard certified under both CC and FIPS 140-2, the \textit{Athena IDProtect}. Its authors used information from CC and FIPS 140-2 certificates to report on the affected certified products, using manual analysis of the certificate reports and security target documents.

The authors report a single vulnerable CC certificate for the \textit{Athena IDProtect} smartcard with ID \href{https://seccerts.org/cc/fca98ecd003e1b82/}{ANSSI-CC-2012/23}. A concrete affected certificate could be identified as its certification report included the CPLC (Card Production Life Cycle) data that matched the data on the vulnerable smartcard. The authors also report on the root cause of the vulnerability as being in another certified item, the \textit{Atmel Cryptographic Toolbox 00.03.11.05} with certificate ID \href{https://seccerts.org/cc/49b4531177e9c3af/}{DCSSI-2009/11}. The vulnerable card's certificate references this certificate. Its security target describes two sets of functions for performing elliptic curve cryptography operations, \textit{secure} and \textit{fast}, with the fast functions not offering any SPA/DPA protection. As the authors note, it is likely that the vulnerable smartcard mistakenly decided to use the fast functions. This sort of root cause analysis would not be possible without using the certification artifacts of CC certificates. 

Using \texttt{sec-certs}, we can search for known vulnerable firmware and its variations using \textit{00.03.11.0\textbf{*}} wildcard, finding another, previously unreported and likely also impacted version \textit{00.03.11.08}. Additionally, the reference graph reveals 32 potentially vulnerable certificates that directly reference those with vulnerable firmware. 

%\textbf{TODO: Add concrete numerical comparison between 1 cert in papers and papers found by seccerts.}
%In the FIPS 140 case, the authors identify several vulnerable certificates starting with certificate \href{https://seccerts.org/fips/f8d64a31eb7d864d/}{\#1711} for the \textit{Athena IDProtect with LASER PKI} smartcard, which again shares the CPLC data with the vulnerable smartcard. The authors then point to NIST's Cryptographic Algorithm Validation Program (CAVP) certificate for ECDSA module 214, which is used in the vulnerable certificate. They then claim that certificates using this module are also affected and list 7 additional certificates. This use of certification metadata again highlights the usefulness of our methodology, using which the search for certificates using a vulnerable module could be entirely automatic.

%\todo[backgroundcolor=green]{JanJ: Add note that we match CVE to one FIPS 140 cert automatically.}

\subsection{Google Titan  (CVE-2021-3011)}
The Side Journey to Titan \cite{titan} paper demonstrated a side-channel attack on ECDSA signing in a chip used in the \textit{Google Titan} security key, as well as in other secure elements and smartcards. While the \textit{Google Titan} security key used the \textit{NXP A7005a} chip, the authors note that directly attacking a commercial secure element with countermeasures in a black-box way is usually really hard. They thus chose to try to get access to a product with the same underlying cryptographic implementation yet with more control:
\textquote{\textit{We went through the public data that can be found online and figured out that several NXP JavaCard smartcards are based on P5x chips and have similar characteristics with the NXP A700X \cite{titan}.}} The authors then performed a similar analysis of CC certification reports as in the case of Minerva, noting:
\blockquote{\textit{Thanks to BSI and NLNCSA CC public certification reports, we were able to gather the following (non-exhaustive) list of NXP JavaCard smartcards based on P5x chips...}}.

The associated CVE-2021-3011\footnote{\url{https://nvd.nist.gov/vuln/detail/CVE-2021-3011}}
%\cite{titan_cve} 
has a listing of vulnerable smartcards. Our \texttt{sec-certs} tool automatically maps the CVE to \numSmartcardsTitanVuln{} CC certificates. Mapping it to the rest of the certificates mentioned in the paper is then a question of looking at the neighborhood of the certificates in the reference graph and perhaps a full-text search query. A re-analysis done using \texttt{sec-certs} found 15 additional certificates referencing the vulnerable cryptographic library (\href{https://seccerts.org/cc/0f684159ad31f883/}{BSI-DSZ-CC-0633-2010}), mostly ePassport products that might be vulnerable.
According to the authors of \cite{titan}, once they validated the attack on NXP JCOP J3D081 and on the Titan key, they spent between half a day to one day manually searching for all the CC certificates of similar products (mainly using the Common Criteria and the BSI website). 
In comparison, our search using the \texttt{sec-certs} tool took 15 minutes. \\

In this section, we revisited four high-profile vulnerabilities and demonstrated how using \texttt{sec-certs} both reduces the time required to perform the vulnerability assessment and leads to a higher number of identified certificates that are affected by the vulnerability. In all cases, incorporating the \texttt{sec-certs} to the researcher's workflow would positively augment the originally achieved results; this comparison is further highlighted in Table~\ref{tab:manual_vs_seccerts}.


\begin{table*}[t]
\captionsetup{font=scriptsize}
\centering
{\scriptsize
\begin{tabular}{ l | c | c | c | c }
    \toprule
    & \multicolumn{2}{c}{\emph{ \# certs. identified }}  &  \multicolumn{2}{c}{\emph{ estimated workload }} \\
    Vulnerability & orig & sec-certs & orig & sec-certs \\
    \midrule
ROCA (CVE-2017-15361) & 32* & 16+119 & not reported & 20 minutes \\
TPM-Fail (CVE-2019-16863) & 1 & 5+7 & not reported & 10 minutes \\
Minerva (CVE-2019-15809) & 2 & 2+32 & 1-2 days & 15 minutes \\
Titan & 11 & 7+15 & 0.5-1 day & 15 minutes \\
    \bottomrule
\end{tabular}
}
\vspace*{0.5em}
\caption{Comparison of the workload and the number of identified vulnerable certificates as reported by the first vulnerability responders in contrast with the analysis done with \emph{sec-certs} tool. Note that in all cases, \texttt{sec-certs} was clearly superior both in the number of identified certificates and in the time required to perform the given task. *Number of certificates from ROCA case was not reported by authors as they were not aware of this resource; full-text search for vulnerable library version '1.02.013' yields 32 certificates.}
\label{tab:manual_vs_seccerts}
\vspace*{-1em}
\end{table*}
